Concolic Testing Heap-Manipulating Programs

Concolic testing is a test generation technique which works effectively by integrating random testing generation and symbolic execution. Existing concolic testing engines focus on numeric programs. Heap-manipulating programs make extensive use of complex heap objects like trees and lists. Testing such programs is challenging due to multiple reasons. Firstly, test inputs for such program are required to satisfy non-trivial constraints which must be specified precisely. Secondly, precisely encoding and solving path conditions in such programs are challenging and often expensive. In this work, we propose the first concolic testing engine called CSF for heap-manipulating programs based on separation logic. CSF effectively combines specification-based testing and concolic execution for test input generation. It is evaluated on a set of challenging heap-manipulating programs. The results show that CSF generates valid test inputs with high coverage efficiently. Furthermore, we show that CSF can be potentially used in combination with precondition inference tools to reduce the user effort.

==> sections/background-symex.tex <==
The term \emph{symbolic execution} refers to a family of techniques that execute a program with symbolic, rather than concrete, input values and compute the effects of the program as {\em functions} in terms of these symbolic inputs.
%For instance, given a program \code{P} with input (or input vector) \code{x}, instead of testing \code{P} with, e.g., \code{x = 3}, SE executes it with a symbol \code{x = X}. At any state \form{\sigma} during the execution of \code{P}, SE keeps two formulas: the symbolic (stack) store \form{\sstack} and the path condition \form{\pc}. \form{\sstack} maps variables to symbolic expressions, and at the initial state \form{\sigma_0}: \code{x \mapsto X}. \form{\pc} records the history of all the branches taken to reach \form{\sigma} from \form{\sigma_0}.
The ``classical'' symbolic execution~\cite{King:1976:SEP:360248.360252,Clarke:1976:SGT:1313320.1313532} uses only symbolic inputs to explore program paths.
%Suppose at the state \form{\sigma} there are branching statement that causes non-deterministic choices, each one is associated with a condition \form{c}. For example, suppose \code{x \mapsto X + 1} in the symbolic store, the conditinal statement \code{x > 5} causes two non-deterministic choices: one with \code{X + 1 > 5} and one with \code{\neg (X+1 > 5)}. For each choice, SE performs case splitting as the following:
%\begin{itemize}
%\item if \form{\pc \rightarrow c}, execute the path associated with $c$ without updating $\pc$,
%\item else if \form{\pc \wedge c} is satisfiable, execute the path associated with $c$, and update \form{\pc \leftarrow \pc \wedge c},
%\item else do not execute the path associated with $c$.
%\end{itemize}
When there is a branching statement \code{if-then-else} with condition \code{c}, classical SE case splits into two branches: the \code{then} branch with the updated path condition \form{\pc_1 \leftarrow \pc \wedge c} and the \code{else} branch with \form{\pc_2 \leftarrow \pc \wedge \neg c}.
These path conditions are checked using off-the-shelf constraint solvers such as Z3~\cite{DeMoura:2008:ZES:1792734.1792766}. If a path condition associated with a branch is not satisfiable, classical SE will stop following that branch.
%For each symbolic path, the solver provides a model that witnesses the satisfiability of \form{\pc}, which is then used as a test input.

A main drawback of classical SE is that it gets stuck or terminates when the constrain solver cannot give a solution within the time limit or if there is external code, e.g. Java native methods, which cannot be symbolically executed. To address these problems, modern symbolic execution engines~\cite{Godefroid:2005:DDA:1065010.1065036,Sen2005,Godefroid:2012:SWF:2090147.2094081} performs mixed \textbf{conc}rete-symb\textbf{olic} execution (and hence the name concolic). When there is branching statement with condition \code{c}, rather than case splitting like classical SE, concolic execution follows the concrete execution to, for example, the \code{then} branch, and updates the path condition \form{\pc_1 \leftarrow \pc \wedge c}. At the end of the execution, it negates a constraint in the path condition, and solve it to generate a new test input, and the execution is re-started from the program entry point.

This design has many advantages over classical SE. When the constraint solver has difficulty solving a path condition, concolic execution can simplify that path condition by concretizing some symbolic variables, i.e. replacing them with their concrete values. Similarly, the variables manipulated by external code or environment can be concretized to obtain a (partial) path condition that can be used to generate test inputs. Moreover, by following a concrete execution and negating the constraints at the end, concolic execution can avoid getting stuck in loops or recursions like classical SE.

Early symbolic execution engines can only handle programs with a fixed number of numerical inputs. In order to apply symbolic execution to programs with data structure inputs,
Khurshid \emph{et al.}~\cite{Khurshid2003} proposed the {\lazy} algorithm that executes programs on inputs with reference variables and fields  being \emph{uninitialized}. When a reference variable or field is first accessed, {\lazy} enumerates all possible heap objects that it can: (i)~be \form{\code{null}}, (ii)~point to a new object with all reference fields being uninitialized, or (iii)~point to any previously initialized object of the same type. By avoiding initializing variables and fields at the beginning, \lazy~can handle inputs from unbounded domains. However, lacking of specification for the input data structures results in the exploration of invalid states and the generation of invalid test cases.


==> sections/prog-syn.tex <==
\input{sections/prog-fig}

